Bayesian uncertainty-weighted loss for improved generalisability on polyp segmentation task

While several previous studies have devised methods for segmentation of polyps, most of these methods are not rigorously assessed on multi-center datasets. Variability due to appearance of polyps from one center to another, difference in endoscopic instrument grades, and acquisition quality result in methods with good performance on in-distribution test data, and poor performance on out-of-distribution or underrepresented samples. Unfair models have serious implications and pose a critical challenge to clinical applications. We adapt an implicit bias mitigation method which leverages Bayesian predictive uncertainties during training to encourage the model to focus on underrepresented sample regions. We demonstrate the potential of this approach to improve generalisability without sacrificing state-of-the-art performance on a challenging multi-center polyp segmentation dataset (PolypGen) with different centers and image modalities.

==> introduction-jr.tex <==
\section{Introduction}

Most gastrointestinal (GI) cancers are preventable. In 2018, the five major types of GI cancers, which include those of the stomach, liver, oesophagus, and colorectum account for 26\% of the global cancer incidence and 35\% of all cancer deaths~\cite{arnold2020global}. Endoscopy, a vital tool for screening and disease surveillance, is however heavily operator dependent and 12\% of cancers are missed~\cite{menon2014commonly}. Artificial intelligence-based systems can play a vital role in improving diagnostic quality. However, it is critical that these tools integrate directly into the existing clinical workflow and generalize well to the previously unseen data. 

Today, high-definition endoscopes provide a sufficient resolution to allow for a detailed visualisation of the mucosal surface. In addition to the conventional white light imaging (WLI) modality, autofluorescence imaging, and electronic chemoendoscopy techniques such as narrow-band imaging have been developed to improve the early detection of cancer and its precursors~\cite{subramanian2014advanced}. It is important that any computer assisted methods should work seamlessly in these different modalities and avoid the need for any modality-specific training. Developing such a modality agnostic approach for detection and segmentation of pre-cancerous changes in the esophagus, and polyps in the lower GI is the focus of this paper.  

\indent{Convolutional} Neural Network (CNN) based approaches~\cite{FCN,Olaf:MICCAI2015,10.1007/978-3-030-01234-2_49}, all  well established in biomedical imaging, have been applied to segmentation tasks in GI endoscopy ~\cite{ALI2021102002,guo2020polyp,wu2021elnet}. Wu et al.~\cite{wu2021elnet} proposed a dual neural network based on U-Net with ResNet backbone for automatic esophageal lesion segmentation. Guo et al.~\cite{guo2020polyp} utilized {a} FCN-based architecture with atrous kernels to segment polyps. However, all these supervised approaches are trained on WLI endoscopy and do not support working in different imaging modalities. 
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\textwidth]{imgs/Fig1.png}
\caption{Example images and masks of the two GI datasets for which source and target domains are separated based on their modality.~\label{fig:1}}
% The top row illustrates the Barrett's esophagus while the bottom row represents the polyps. Here, the left column correspond to white light imaging (WLI) modality which is source domain in our study and the right column demonstrate the narrow band imaging (NBI) modality used as target domain.
\end{figure}
%
To date, the problem of quantifying disease related changes in NBI, which can produce a very different appearance of the mucosal surface when compared to WLI (see Fig.~\ref{fig:1}) has not been addressed. Training methods for different imaging modalities independently is prohibitive. Firstly, extensive training datasets that cover a similar range of conditions would need to be curated to ensure a comparable performance. Secondly, manual annotations by human experts are required which is not only labour intensive but also expensive. 
%
To tackle these issues domain adaptation methods have been used to adapt trained models to unseen target data for segmentation~\cite{Tsai,CardioUDA,pmlr-v121-haq20a,10.1007/978-3-030-58539-6_25}. 
{Although these methods promise to generalise, so far there are only a few examples of applying such methods to medical data ~\cite{CardioUDA,pmlr-v121-haq20a}}. Additionally, the available methods still under-perform and have not been adapted for extremely diverse modality cases such as that in the GI endoscopy. 

%Tsai et al.~\cite{Tsai} developed a domain adaptation model for semantic segmentation based on a multi-level adversarial network that shares the segmentation loss for both source and target domains. In the discriminator network, target domain predictions are matched to the source domain predictions whether the input is from the source or target domain via an adversarial loss. In the context of biomedical image segmentation, Dong et al.~\cite{CardioUDA} proposed an unsupervised domain adaptation (UDA) technique for cardiothoracic ratio estimation by performing domain invariant chest organ segmentation. Haq et al.~\cite{pmlr-v121-haq20a} introduced an alternative UDA framework that included a decoder network to reconstruct the input images for cell segmentation. Pandey et al.~\cite{10.1007/978-3-030-58539-6_25} employed UDA approach to segment human skin under different imaging modalities via a variational auto-encoder (VAE) based generative model.
%

To develop a modality-agnostic approach, we propose to use an unsupervised domain adaptation (UDA) technique that can be trained on available single WLI modality dataset and can be applied on an unseen NBI imagery. For such settings, where classical supervised models fail to generalize and perform poorly, we show that our proposed target-independent UDA technique, EndoUDA, has the potential to generalize and {to} provide improved segmentation on NBI modality for both BE and polyp datasets. 
%


==> introduction-old.tex <==
Esophageal adenocarcinoma (EAC) is the seventh most common cause of cancer deaths with 14\% five years survival rate while colorectal cancer (CRC) has the third highest mortality rate with overall five-year survival rate of only around 68\%. One common early precursor of EAC is the Barrett's oesophagus (BE) in esophagus~\cite{cook2018cancer} and polyp in the CRC~\cite{holme2013flexible}. Changes in the surface color (e.g., changes in color of the mucosa in BE, see Fig.~\ref{fig:1} (top)) and the surface topology (e.g., protrusion of mucosa, see Fig.~\ref{fig:1} (bottom)) of the tissue and other irregularities indicate precancerous changes. Studies have shown that population-wide screening and quantification can advance the prognosis and can even reduce the incidences~\cite{holme2013flexible}. Endoscopy is the standard tool for both diagnostic and therapeutic procedures for reducing risks of such occurrences. It is thus imminently important to quantify these areas accurately and monitor these changes. While manual comparison of these areas is difficult to perform, automated segmentation methods can help in to obtain more accurate and measurable quantification of these areas. 

Today, there are many such methods built for segmentation of such areas but most of these methods require abundant amount of annotations. It is evident that manual segmentation of specialized medical conditions such as BE and polyp are prone to human subjectivity and require extensive knowledge in clinical endoscopy. Additionally, such processes are labor intensive due to the large annotation time required for pixel-wise delineation of such areas in these images. Due to the high risk associated with these cancer precursors, often complimentary modality such as narrow-band imaging (NBI) is widely used in addition to the conventional white-light imaging (WLI) modality. While, most automated methods for segmentation are based on the WLI modality, no work is done in direction of quantifying NBI modality which can produce a very diverse set of images as shown in Fig.~\ref{fig:1} compared to WLI. The lack of abundant and curated NBI dataset is a major bottleneck for applying supervised techniques. Additionally, curating modality specific dataset will require an additional enormous amount of time from clinical experts. To mitigate such problems, we propose to use unsupervised domain adaptation (UDA) technique that can be trained on available single WLI modality dataset and can be applied on an unseen NBI modality dataset. For such settings, where classical supervised models fail to generalize and perform poorly, we show that our proposed UDA technique has the potential to generalize and provide improved segmentation on NBI modality for both BE and polyp datasets. 

\indent{Convolutional} Neural Network (CNN) based approaches such as Fully Convolutional Network (FCN)~\cite{FCN}, U-Net~\cite{Olaf:MICCAI2015}, DeepLab~\cite{10.1007/978-3-030-01234-2_49} are known to perform well in the biomedical image segmentation domain, including segmentation tasks on gastrointestinal (GI) endoscopy~\cite{ALI2021102002,guo2020polyp,wu2021elnet,mendel2017barrett}. Wu et al.~\cite{wu2021elnet} proposed a dual neural network based on U-Net with ResNet backbone for automatic esophageal lesion segmentation. Similarly, majority of the teams in the multi-class GI disease segmentation challenge~\cite{ALI2021102002} also used U-Net-based models. Guo et al.~\cite{guo2020polyp} utilized FCN-based architecture with atrous kernels to segment polyps. All of these supervised methods are built on a single WLI modality endoscopy. However, in clinical endoscopy, endoscopists often use other complimentary modalities such as widely used NBI to characterize the tissue. Due to the incapability of these fully supervised models to generalize well to different imaging modalities due to domain shift, and lack of reliable and bulk annotations required by supervised models for each specific modality; there has not been much work done towards solving this problem in medical imaging domain. In this context, domain adaptation~\cite{ADDA} approaches have been proposed for unsupervised or semi-supervised domain learning wherein annotations are not required in the target (test) dataset consisting of a different imaging modality or dataset. 

Tsai et al.~\cite{Tsai} developed a domain adaptation model for semantic segmentation based on a multi-level adversarial network that shares the segmentation loss for both source and target domains. In the discriminator network, target domain predictions are matched to the source domain predictions whether the input is from the source or target domain via an adversarial loss. In the context of biomedical image segmentation, Dong et al.~\cite{CardioUDA} proposed an unsupervised domain adaptation (UDA) technique for cardiothoracic ratio estimation by performing domain invariant chest organ segmentation. Haq et al.~\cite{pmlr-v121-haq20a} introduced an alternative UDA framework that included a decoder network to reconstruct the input images for cell segmentation. Pandey et al.~\cite{10.1007/978-3-030-58539-6_25} employed UDA approach to segment human skin under different imaging modalities via a variational auto-encoder (VAE) based generative model. The existing GI endoscopy image segmentation methods are however limited by the fully supervised methods~\cite{ALI2021102002,guo2020polyp,wu2021elnet}. 

To the best of our knowledge, this is the first work that exploits the learned latent vector space representation in the VAE obtained from the source domain (WLI) to generalize to segment unseen target (NBI) dataset in GI endoscopy. Our novel EndoUDA utilizes a simplified architecture compared to the state-of-the-art GLSS method~\cite{10.1007/978-3-030-58539-6_25}. Our architecture includes the utilization of a common EfficientNet-B4 backbone for both U-Net and VAE encoder, and a weighted loss function for faster convergence of target latent space projection during inference. Our contributions can be summarised as follows: 1) Unsupervised domain adaptation approach (EndoUDA) based on generative model for the segmentation of GI endoscopy anomalies for unseen NBI modality, 2) simplified network with shared encoder for VAE and segmentation modules, 3) a weighted loss for achieving optimal nearest clone of target image during inference, 4) a comprehensive comparison of the state-of-the-art baseline methods showing efficacy of our proposed method, and 5) ablation studies showing evidences for improvement of our proposed model design.
